Using Model-Checking Techniques for Component-Based Systems with Reconfigurations

Within a component-based approach allowing dynamic reconfigurations, sequences of successive reconfiguration operations are expressed by means of reconfiguration paths, possibly infinite. We show that a subclass of such paths can be modelled by finite state automata. This feature allows us to use techniques related to model-checking to prove some architectural, event, and temporal properties related to dynamic reconfiguration. Our method is proved correct w.r.t. these properties' definition.

==> babelbst.tex <==
%%  Putting default values for bibliographic keywords:

\makeatletter

\expandafter\ifx\csname l@english\endcsname\relax\else%
 \addto{\extrasenglish}{%
   %%  Months:
  \def\bbljan{January}%
  \def\bblfeb{February}%
  \def\bblmar{March}%
  \def\bblapr{April}%
  \def\bblmay{May}%
  \def\bbljun{June}%
  \def\bbljul{July}%
  \def\bblaug{August}%
  \def\bblsep{September}%
  \def\bbloct{October}%
  \def\bblnov{November}%
  \def\bbldec{December}%
  %%  Ordinal numbers:
  \def\bblfirsto{1st}%
  \def\bblsecondo{2nd}%
  \def\bblthirdo{3rd}%
  \def\bblfourtho{4th}%
  \def\bblfiftho{5th}%
  \def\bblst{st}%
  \def\bblnd{nd}%
  \def\bblrd{rd}%
  \def\bblth{th}%
  %%  Other keywords:
  \def\bbland{and}%
  \def\bblchap{chap.}%
  \def\bbled{ed.}%
  \def\bbledby{ed.\ by}%
  \def\bbledn{edition}%
  \def\bbleds{eds.}%
  \def\bblin{in}%
  \def\bblmthesis{Master's thesis}%
  \def\bblno{no.}%
  \def\bblof{of}%
  \def\bblp{p.}%
  \def\bblphdthesis{PhD thesis}%
  \def\bblpp{p.}%
  \def\bbltechrep{Technical Report}%
  \def\bblvol{Vol.}%
  \def\bblwith{with}%
  %%  Quoting some titles in bibliographies:
  \def\bblquotedtitle{``}%
  \def\endbblquotedtitle{\unskip''}}%
\fi

\expandafter\ifx\csname l@frenchb\endcsname\relax\else%
 \addto{\extrasfrench}{%
  %%  Months:
  \def\bbljan{Janvier}%
  \def\bblfeb{F\'{e}vrier}%
  \def\bblmar{Mars}%
  \def\bblapr{Avril}%
  \def\bblmay{Mai}%
  \def\bbljun{Juin}%
  \def\bbljul{Juillet}%
  \def\bblaug{Ao\^{u}t}%
  \def\bblsep{Septembre}%
  \def\bbloct{Octobre}%
  \def\bblnov{Novembre}%
  \def\bbldec{D\'{e}cembre}%
  %%  Ordinal numbers:%
  \def\bblfirsto{1\up{re}}%
  \def\bblsecondo{2\up{e}}%
  \def\bblthirdo{3\up{e}}%
  \def\bblfourtho{4\up{e}}%
  \def\bblfiftho{5\up{e}}%
  \def\bblst{\up{er}}%
  \def\bblnd{\up{e}}%
  \def\bblrd{\up{e}}%
  \def\bblth{\up{e}}%
  %%  Other keywords:
  \def\bbland{et}%
  \def\bblchap{chap.}%
  \def\bbledn{\'{e}dition}%
  \def\bbled{r\'{e}dacteur en chef}%
  \def\bbledby{dirig\'{e} par}%
  \def\bbleds{r\'{e}dacteurs en chef}%
  \def\bblin{\emph{in}}%
  \def\bblmasterthesis{M\'{e}moire}%
  \def\bblno{n\textsuperscript{o}}%
  \def\bblof{de}%
  \def\bblp{p.}%
  \def\bblpp{p.}%
  \def\phdthesis{Th\`{e}se}%
  \def\bbltechrep{Rapport technique}%
  \def\bblvol{Vol.}%
  \def\bblwith{avec}%
  %%  Quoting some titles in bibliographies:
  \def\bblquotedtitle{\og}%
  \def\endbblquotedtitle{\fg}}%
\fi

\expandafter\ifx\csname l@german\endcsname\relax\else%
 \addto{\extrasgerman}{%
  %%  Months:
  \def\bbljan{Januar}%
  \def\bblfeb{Februar}%
  \def\bblmar{M\"{a}rz}%
  \def\bblapr{April}%
  \def\bblmay{Mai}%
  \def\bbljun{Juni}%
  \def\bbljul{Juli}%
  \def\bblaug{August}%
  \def\bblsep{September}%
  \def\bbloct{Oktober}%
  \def\bblnov{November}%
  \def\bbldec{Dezember}%
  %%  Ordinal numbers:
  \def\bblfirsto{1.}%
  \def\bblsecondo{2.}%
  \def\bblthirdo{3.}%
  \def\bblfourtho{4.}%
  \def\bblfiftho{5.}%
  \def\bblst{.}%
  \def\bblnd{.}%
  \def\bblrd{.}%
  \def\bblth{.}%
  %%  Other keywords:
  \def\bbland{und}%
  \def\bblchap{Kap.}%
  \def\bbled{Chefredakteur}%
  \def\bbledby{\relax}%
  \def\bbledn{Auflage}%
  \def\bbleds{Chefredakteure}%
  \def\bblin{\emph{in}}%
  \def\bblmasterthesis{\relax}%
  \def\bblno{Nr.}%
  \def\bblof{in}%
  \def\bblp{S.}%
  \def\bblphdthesis{\relax}%
  \def\bblpp{S.}%
  \def\bbltechrep{Technischer Bericht}%
  \def\bblvol{Bd.}%
  \def\bblwith{mit}%
  %%  Quoting some titles in bibliographies:
  \def\bblquotedtitle{\glqq}%
  \def\endbblquotedtitle{\unskip\grqq}}%
\fi

\expandafter\ifx\csname l@portuges\endcsname\relax\else%
 \addto{\extrasportuges}{%
   %%  Months:
  \def\bbljan{January}%
  \def\bblfeb{February}%
  \def\bblmar{March}%
  \def\bblapr{April}%
  \def\bblmay{May}%
  \def\bbljun{June}%
  \def\bbljul{July}%
  \def\bblaug{August}%
  \def\bblsep{September}%
  \def\bbloct{October}%
  \def\bblnov{November}%
  \def\bbldec{December}%
  %%  Ordinal numbers:
  \def\bblfirsto{1st}%
  \def\bblsecondo{2nd}%
  \def\bblthirdo{3rd}%
  \def\bblfourtho{4th}%
  \def\bblfiftho{5th}%
  \def\bblst{st}%
  \def\bblnd{nd}%
  \def\bblrd{rd}%
  \def\bblth{th}%
  %%  Other keywords:
  \def\bbland{and}%
  \def\bblchap{chap.}%
  \def\bbled{ed.}%
  \def\bbledby{ed.\ by}%
  \def\bbledn{edition}%
  \def\bbleds{eds.}%
  \def\bblin{in}%
  \def\bblmthesis{Master's thesis}%
  \def\bblno{no.}%
  \def\bblof{of}%
  \def\bblp{p.}%
  \def\bblphdthesis{PhD thesis}%
  \def\bblpp{p.}%
  \def\bbltechrep{Technical Report}%
  \def\bblvol{Vol.}%
  \def\bblwith{with}%
  %%  Quoting some titles in bibliographies:
  \def\bblquotedtitle{``}%
  \def\endbblquotedtitle{\unskip''}}%
\fi

\select@language{\languagename}

\makeatother

%%%  End of file "babelbst.tex"


==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v{n} (Eds.):\\
Formal Engineering approaches to Software\\
Components and Architectures (FESCA'15).\\
EPTCS 178, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.178.4}{10.4204/EPTCS.178.4}}
\pdfoutput=1

